Kafka Consumer Group Autoscaler

Message brokers enable asynchronous communication between data producers and consumers in distributed environments by assigning messages to ordered queues. Message broker systems often provide with mechanisms to parallelize tasks between consumers to increase the rate at which data is consumed. The consumption rate must exceed the production rate or queues would grow indefinitely. Still, consumers are costly and their number should be minimized. We model the problem of determining the required number of consumers, and the partition-consumer assignments, as a variable item size bin packing variant. Data cannot be read when a queue is being migrated to another consumer. Hence, we propose the R-score metric to account for these rebalancing costs. Then, we introduce an assortment of R-score based algorithms, and compare their performance to established heuristics for the Bin Packing Problem for this application. We instantiate our method within an existing system, demonstrating its effectiveness. Our approach guarantees adequate consumption rates something the previous system was unable to at lower operational costs.

==> appendices/modified_any_fit.tex <==

\section{Modified Any Fit Algorithm}



==> sections/old.tex <==

With the goal of testing the system as a whole, we statistically summarize the
time it takes the autoscaler to go through each event required to dynamically
scale the group of consumers.  

\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.95\columnwidth]{images/pdf/Integration_diagram.pdf}
    \caption{System sequence of events.}
\label{fig:step_event_sequence}
\end{figure}

Initially, a measurement has to be provided by the monitor process to then be
consulted by the controller ($\Delta_{t1}$). The controller then updates the
group's current state based on the new measurement, and proceeds to computing a
new group configuration using one of the heuristic algorithms presented in
Sections \ref{sub:approximation_algorithms} and \ref{sub:modified_any_fit}. This is followed by the controller calculating the
difference between the new and current configuration, to determine the consumers
it has to create, the ones it has to delete, and the messages that have to be
communicated to each consumer to reach the intended state (Section
\ref{autoscaler:controller}). This step terminates with the controller
communicating with the Kubernetes control plane, to create the new consumer
resources ($\Delta_{t2}$). 

The controller then waits for the newly created deployments to be ready
($\Delta_{t3}$), followed by communicating with the consumer group to inform the
consumers of their change in state, which only terminates as
soon as all messages have been sent out to the respective consumers, and when every message
has been acknowledged back to the controller ($\Delta_{t4}$). This process is illustrated
by Figure \ref{fig:step_event_sequence}.

To accurately determine the time it takes the monitor process to converge to the
real produced speed ($\Delta_{t1}$), we used 31 different step values as input,
created by a producer that sends data at a constant rate to a given partition.
As expected, Fig. \ref{fig:controller_result_monitor} shows the monitor process
takes approximately 30 seconds, related to the fact that the monitor computes an
average write speed over the last 30 seconds.

\begin{figure}[!htb]
\centering
\includegraphics[width=0.9\columnwidth]{images/integration/delta1.png}
\caption{
    Distribution of $\Delta_{t1}$ for 31 different step inputs.
}
\label{fig:controller_result_monitor}
\end{figure}

As for the second event $\Delta_{t2}$, this is the time it takes the controller
to compute the consumer group's new assignment, computing the difference between
the new and current states, and to send an asynchronous request to the Google
Kubernetes Engine (GKE) cluster for every new consumer instance to be created.
To obtain the distribution for this metric, the system was tested with the
aforementioned step inputs and the randomly generated streams described in Sec.
\ref{sec:random_data_generation}.

\begin{figure}[htb!]
\centering
\includegraphics[width=0.9\columnwidth]{images/integration/delta2.png}
\caption{
    Distribution of $\Delta_{t2}$ for 1345 observations.
}
\label{fig:controller_result_trigger}
\end{figure}

The time the controller takes with this procedure depends on the number of
partitions to distribute between the consumer group, the algorithm the
controller is executing to figure a new consumer group assignment, and the
number of new consumer instances it has to create in the GKE cluster.

For the tested input data, there were at most 32 partitions to rebalance, at
most 20 consumers to be created in a single iteration and the algorithm executed
was the MWF. The event consistently takes less than 1 second to be executed as
shown in Figure \ref{fig:controller_result_trigger}.

After making the asynchronous request to the GKE cluster, the autoscaler enters
$\Delta_{t3}$, where it has to wait for the control plane to schedule the
consumer pods to cluster nodes, and run the containers.

From Fig. \ref{fig:controller_result_kubernetes}, there are two main clusters of
data points which can be summarized into two different scenarios in which the
GKE cluster can find itself in.

\begin{figure}[htb!]
\centering
\includegraphics[width=0.9\columnwidth]{images/integration/delta3.png}
\caption{
    Histogram of $\Delta_{t3}$ for 273 observations.
}
\label{fig:controller_result_kubernetes}
\end{figure}

The first, and most frequent (88\%), has the GKE cluster taking between $[10,
50]$ seconds to have a new consumer instance ready. This is usually the case
when the controller requests for the creation of new consumer instances and the
Kubernetes cluster has enough resources available. As such, the event's duration
is related to the time it takes the scheduled node(s) to download the image from
the container registry, and to start the containers.

The second group of data points, any time span greater than $50s$ (represents
12\% of the data points), occurs when the Kubernetes cluster does not have any
available resources. Here the actions the cluster undergoes are adding a new
node to the cluster, and only then scheduling the consumer instance into the new
available node. Due to the autoscaling feature of the GKE cluster, this is done
automatically but it is also more inconsistent, having data points taking up to
$500s$, although very sporadically.

In spite the fact there isn't much control over the time it takes the Kubernetes cluster to schedule and start the pods, one variable that can be controlled is the size of the image which has to be downloaded by the nodes that were assigned the newly created consumer instances.

Lastly, after having the consumer instances running and ready to receive
assignments, the controller has to communicate each consumer's assignment
within the newly computed group configuration, which is represented by
$\Delta_{t4}$ in Fig. \ref{fig:controller_result_change_state}. 

Due to the synchronous nature of rebalancing a partition from one consumer to
another, the controller has to first send out a stop consuming message for each
of these partitions, wait for the consumer to respond, send out a start
consuming message, and wait for a response. Without taking into account any
processing and network delays, at worst, the controller might have to wait for
two consumer cycles to be able to rebalance a partition. 

\begin{figure}[htb!]
\centering
\includegraphics[width=0.9\columnwidth]{images/integration/delta4.png}
\caption{
    Distribution of $\Delta_{t4}$ for 1331 observations.
}
\label{fig:controller_result_change_state}
\end{figure}

A consumer's cycle goes through the different phases mentioned in Section
\ref{sub:consumer}, and only after performing it's tasks does it verify
the metadata queue to check if it has received any change in state message. For
this reason, between two metadata reads from the $consumer.metadata$
topic, it takes the consumer one whole cycle. 

Having defined $BATCH\_BYTES$ to be 5 seconds and
$WAIT\_TIME\_SECS$ 1 second, and provided the results from Figure
\ref{fig:consumer_capacity}, which indicate the consumer has a maximum
consumption rate of approximately $2Mbytes/s$, each consumer cycle can take
approximately $2.5s$.  Since the controller has to wait for two consumer cycles,
this would imply that changing the group's state could take around 5 seconds, as
can be seen in Fig. \ref{fig:controller_result_change_state}.

It is also worth noting that the more consumers there are in the group, the
higher the probability that the controller has to wait 1 whole cycle after
sending out the stop command, and another whole cycle after a start command, as
the communication would have to be performed with more consumers.

